Parameter-Efficient Mixture-of-Experts Architecture for Pre-trained Language Models

Recently, Mixture-of-Experts (short as MoE) architecture has achieved remarkable success in increasing the model capacity of large-scale language models. However, MoE requires incorporating significantly more parameters than the base model being extended. In this paper, we propose building a parameter-efficient MoE architecture by sharing information among experts. We adopt the matrix product operator (MPO, a tensor decomposition from quantum many-body physics) to reconstruct the parameter matrix in the expert layer and increase model capacity for pre-trained language models by sharing parameters of the central tensor (containing the core information) among different experts while enabling the specificity through the auxiliary tensors (complementing the central tensor) of different experts. To address the unbalanced optimization issue, we further design the gradient mask strategy for the MPO-based MoE architecture. Extensive experiments based on T5 and GPT-2 show improved performance and efficiency of the pre-trained language model (27.2x reduction in total parameters for the superior model performance, compared with the Switch Transformers). Our code is publicly available at https://github.com/RUCAIBox/MPOE.

==> appd.tex <==
\appendix

We offer some proof as supplementary materials to help reviewers better understand our model. The appendix includes \underline{4 pages} and is organized into sections:
\begin{itemize}
    \item MPO and MoE Details
    \item Theorem
    \item Experiment Details
    \item More Discussion
    \item Maximum Mean Discrepancy among Experts
\end{itemize}



\section{Matrix Product Operators and Mixture-of-Experts}


\paratitle{Definition 1} \\
(Matrix product operator).
We present a detailed algorithm for MPO decomposition in Algorithm~\ref{alg:mpo-decomposition}.
The $k$-th order~\cite{kolda2009tensor} and $k\in\{1,\dots,D\}$.
The bond dimension $d_k$ is defined by:
\begin{equation}
    d_k = \min\bigg(\prod_{m=1}^k i_m\times j_m, \prod_{m=k+1}^n i_m\times j_m\bigg).
    \label{eq:d-k}
\end{equation}
From Eq.~\eqref{eq:d-k}, we can see that is going to be large in the middle and small on both sides. We present a detailed algorithm for MPO decomposition in Algorithm~\ref{alg:mpo-decomposition}.

\floatname{algorithm}{Algorithm}
\begin{algorithm}
\small
    \caption{MPO decomposition procedure.}   
    \begin{algorithmic}[1] %每行显示行号
        \Require matrix 
        $\Matrix{M}\in \mathbb{R}^{I\times J}$, the number of local tensor $n$
        \Ensure: local tensor set $ \{\Tensor{T}_{(k)}\}_{k=1}^{n}$
        \For{$k=1,\dots,n-1$ }
            \State $\Matrix{M}[d_{k-1}\times i_k\times j_k,-1] = \rm{Reshape}(\Matrix{M}[I,J])$
            \State \ $\Matrix{U}\lambda \Matrix{V}^\top=\rm{SVD}~(\Matrix{M})$
            \State $\Tensor{U}[d_{k-1},i_k,j_k,d_k] = \rm{Reshape}(\Matrix{U})$
            \State Let \ $\Tensor{T}^{(k)}= \Tensor{U} $
            \State Calculate \ $\Matrix{M}= \lambda \Matrix{V}^{\top}$
        \EndFor
        \State Let $\Tensor{T}^{(n)} =\Matrix{M}$
        \State $\rm{Normalization}$
        \State \Return{${\rm{local\ tensor\  set\ }} \{\Tensor{T}_{(k)}\}_{k=1}^{n}$}
    \end{algorithmic}
\label{alg:mpo-decomposition}
\end{algorithm}

With Eq.~\eqref{Eq:MPO} we can decompose an original matrix $\Matrix{M}$ to a sequential product of the derived local tensors.



The MPO representation of $\Matrix{M}$ is obtained by factorizing it into a sequential product of local tensors. The algorithm has been depicted in Section 3 of the main text.
With MPO decomposition technique, we can get local tensor as follows:
\begin{eqnarray}
 \Matrix{M}_{i_1\cdots i_n,j_1\cdots j_n} =  \Tensor{T}^{(1)} [i_1,j_1] \cdots \Tensor{T}^{(n)} [i_n,j_n]  \label{Eq:MPO}
\end{eqnarray}
where $\Tensor{T}^{(k)}[j_k,i_k]$ is a $D_{k-1}\times D_{k}$ matrix with $D_k$ the virtual basis dimension on the bond linking $\Tensor{T}^{(k)}$ and $\Tensor{T}^{(k+1)}$ with $D_0=D_n=1$.

\paratitle{Mixture-of-Experts~(MoE)}
An MoE model consists of a set of $N$ ``expert networks'' $E_1,...,E_N,$ and a ``gating network'' $G$ whose output is a sparse $N$-dimensional vector. Experts usually use feed-forward sub-networks~(FFN), each with identical architectures but separate parameters. 
Let  $G(x)$ and $E_i(x)$ denote the output vector of the gating network and the output of the $i$-th expert network for a given input $x$, respectively. 
The  output of MoE model $y$ can be expressed as:
\begin{equation}
    y=\sum_{i=1}^{N}G(x)_i \cdot E_i(x).
    \label{eq:moe-out1}
\end{equation}

The $\rm{softmax}$ function is widely used as the gating function $G(x)$ that is randomly initialized.
The sparse-gated MoE model, which used a noisy top-$k$ gating mechanism to reduce computational cost, was proposed in~\citep{shazeer2017outrageously}.
It adds tunable Gaussian noise with $H(\cdot)$, then keep only the top-$k$ values with $\rm{KeepTopK}(\cdot)$, setting the rest $-\infty$. This keeps only the top $k$ experts to be evaluated with $G(x)=\textrm{\rm{softmax}(\rm{KeepTopK}}(H(x),k))$.
Furthermore, switch transformer uses switch routing strategy to simplify this gating function by routing to a \emph{single} expert~\citep{fedus2021switch}. 
\section{Theorem}

\begin{thm}\label{thm1}
Suppose that the tensor $\textbf{W}^{(k)}$ of matrix $W$ that is satisfy 
\begin{align}
    &\Matrix{W} = \Matrix{W}^{(k)} + \Matrix{E}^{(k)}  ,D( \textbf{W}^{(k)}) = d_k,\notag\\
    &where\quad||\Matrix{E}^{(k)}||_F^2 = \epsilon_k^2 , k = 1,...,d-1. 
\end{align}
Then MPO$(\Matrix{W})$ with the $k$-th bond dimension $d_k$ upper bound of truncation error satisfy:
\begin{equation}
    ||\Matrix{W}-{\rm{MPO}}~(\Matrix{W})||_F \leq \sqrt{\sum_{k=1}^{d-1} \epsilon_k^2}
\end{equation}
\end{thm}

$Proof.$ The proof is by induction. For $n = 2$ the statement follows from the properites of the SVD. Consider an arbitrary $n > 2$. Then the first unfolding $\Matrix{W}^{(1)}$ is decomposed as
\begin{equation}
    \Matrix{W}^{(1)} = \Matrix{U}_1 \Matrix{\lambda}_1 \Matrix{V}_1 + \Matrix{E}^{(1)} = \Matrix{U}_1\Matrix{B}^{(1)} + \Matrix{E}^{(1)},
\end{equation}
where $\Matrix{U}_1$ is of size $r_1\times i_1 \times j_1$ and $|| \Matrix{E}^{(1)}||_F^2 = \epsilon_1^2$. The matrix $\Matrix{B}_1$ is naturally associated with a $(n-1)$-dimensional tensor $\Tensor{B}^{(1)}$ with elements $\Tensor{B}^{(1)}(\alpha , i_2,j_2, ..., i_n,j_n)$, which will be decomposed further. This means that $\Matrix{B}_1$ will be approximated by some other matrix $\hat{\Matrix{B}_1}$. From the properties of the SVD it follows that $\Matrix{U}_1^{T}\Matrix{E}^{(1)}=0$, and thus

\begin{align}
    & ||\Matrix{W}-\Tensor{B}^{(1)}||^2_F \notag\\ 
    & = ||\Matrix{W}_1 - \Matrix{U}_1\hat{\Matrix{B}_1}||_F^{2} \notag\\
    & = ||\Matrix{W}_1 - \Matrix{U}_1(\hat{\Matrix{B}_1} + \Matrix{B}_1 - \Matrix{B}_1)||_F^{2}\notag\\
    & = ||\Matrix{W}_1 - \Matrix{U}_1\Matrix{B}_1||_F^{2} + ||\Matrix{U}_1(\hat{\Matrix{B}_1} - \Matrix{B}_1)||_F^2
\end{align}


and since $\Matrix{U}_1$ has orthonormal columns,
\begin{equation}
    ||\Matrix{W}-\Tensor{B}^{(1)}||_F^2 \leq \epsilon_1^2 + ||\Matrix{B}_1-\hat{\Matrix{B}_1}||_F^2.
    \label{eq:thm1}
\end{equation}
and thus it is not difficult to see from the orthonormality of columns of $\Matrix{U}_1$ that the distance of the $k$-th unfolding $(k=2,...,d_k-1)$ of the $(d-1)$-dimensional tensor $\Tensor{B}^{(1)}$ to the $d_k$-th rank matrix cannot be larger then $\epsilon_k$. Proceeding by induction, we have 
\begin{equation}
    ||\Matrix{B}_1 - \hat{\Matrix{B}_1} ||_F^2 \leq \sum_{k=2}^{d-1} \epsilon_k^2,
\end{equation}
combine with Eq.~\eqref{eq:thm1}, this complets the proof.



\section{Experiment Details}
\label{appendix-exp}
\subsection{Details of Datasets and Metrics}
\paratitle{Datasets.}
For the language modeling task, we use text in widely used WikiText-2~\cite{wikitext}, a small preprocessed version of Wikipedia. For the text generation task, we use IMDB~\cite{imdb} and EMNLP2017 WMT News~\cite{EMNLPnews} as long and short corpus respectively. IMDB movie review dataset consists of 25K/25K train/test movie review comments with a maximum length of 2956, while EMNLP2017 WMT News consists of 270K/10K train/test sentences with a maximum length of 51. 

GLUE benchmark covers multiple datasets (MRPC, QQP, SST-2, MNLI, RTE, QNLI, CoLA)\footnote{Following~\cite{multitask2020raffel}, as a common practice, due to the adversarial nature of WNLI with respect to the training set, we do not experiment with WNLI}. The original test sets are not publicly available, and following~\cite{fewsample2021zhang}, for datasets fewer than 10$K$ samples~(RTE, MRPC, STS-B, CoLA), we divide the original validation set in half, using one half for validation and the others for the test.

\paratitle{Metrics.}
We use perplexity~(PPL)~\cite{DBLP:journals/coling/BrownPPLM92} to measure how well the probability model predicts a sample compared with the ground-truth. To evaluate the ratios of the overlapping $n$-grams between generated and real samples, we use BLEU-$n$ score~\cite{DBLP:conf/acl/PapineniRWZ02}. We also take into account the Self-BLEU-$n$ score~\cite{DBLP:conf/sigir/ZhuLZGZWY18} to evaluate the diversity of generated samples especially.
For metrics used in the GLUE benchmark, we follow~\cite{rabeeh2021hyperformer} and use Matthew's correlation for CoLA, Pearson for STS-B, and accuracy for the other tasks.

\subsection{Additional Details of MPO}
\label{sec:additional-details}
In this paper, the MPOE is proposed to effectively increase model capacity based on MPO decomposition. In order to show that the process of incorporating several MPO structures into T5-based and GPT-based pre-trained language models respectively, we introduce MPO decomposition in T5 and GPT details as follows:

\begin{table}[ht]
\small
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lll}
\toprule[1pt]
Layers                          & Matrix shape               & \begin{tabular}[c]{@{}l@{}}\multirow{1}{*}{MPO shape} \\ {[$d_{k-1},i_k,j_k,d_k$]}\end{tabular} \\ \midrule[0.7pt]
\multirow{10}{*}{\makecell{T5-base}} & \multirow{5}{*}{$768\times3072$}  & $\Tensor{A}_1$:$[1,3,4,12]$                \\
                                &                            & $\Tensor{A}_2$:$[12,4,4,192]$              \\
                                &                            & $\Tensor{C}$:$[192,4,8,384]$              \\
                                &                            & $\Tensor{A}_3$:$[384,4,6,16]$              \\
                                &                            & $\Tensor{A}_4$:$[16,4,4,1]$                \\\cline{2-3}
                                & \multirow{5}{*}{$3072\times768$}  & $\Tensor{A}_1$:$[1,4,3,12]$                \\
                                &                            & $\Tensor{A}_2$:$[12,4,4,192]$              \\
                                &                            & $\Tensor{C}$:$[192,8,4,384]$              \\
                                &                            & $\Tensor{A}_3$:$[384,6,4,16]$              \\
                                &                            & $\Tensor{A}_4$:$[16,4,4,1]$                \\ \midrule
\multirow{10}{*}{\makecell{T5-large}} & \multirow{5}{*}{$1024\times4096$}  & $\Tensor{A}_1$:$[1,4,4,16]$                \\
                                &                            & $\Tensor{A}_2$:$[12,4,4,256]$              \\
                                &                            & $\Tensor{C}$:$[256,8,4,512]$              \\
                                &                            & $\Tensor{A}_3$:$[512,4,8,16]$              \\
                                &                            & $\Tensor{A}_4$:$[16,4,4,1]$                \\\cline{2-3}
                                & \multirow{5}{*}{$4096\times1024$}  & $\Tensor{A}_1$:$[1,4,4,16]$                \\
                                &                            & $\Tensor{A}_2$:$[16,4,4,256]$              \\
                                &                            & $\Tensor{C}$:$[256,8,4,512]$              \\
                                &                            & $\Tensor{A}_3$:$[512,8,4,16]$              \\
                                &                            & $\Tensor{A}_4$:$[16,4,4,1]$                \\ \midrule
\multirow{10}{*}{\makecell{GPT2}} & \multirow{5}{*}{$768\times3072$}  & $\Tensor{A}_1$:$[1,3,4,12]$                \\ 
                                &                            & $\Tensor{A}_2$:$[12,4,4,192]$              \\
                                &                            & $\Tensor{C}$:$[192,4,8,384]$              \\
                                &                            & $\Tensor{A}_3$:$[384,4,6,16]$              \\
                                &                            & $\Tensor{A}_4$:$[16,4,4,1]$                \\\cline{2-3}
                                & \multirow{5}{*}{$3072\times768$}  & $\Tensor{A}_1$:$[1,4,3,12]$                \\
                                &                            & $\Tensor{A}_2$:$[12,4,4,192]$              \\
                                &                            & $\Tensor{C}$:$[192,8,4,384]$              \\
                                &                            & $\Tensor{A}_3$:$[384,6,4,16]$              \\
                                &                            & $\Tensor{A}_4$:$[16,4,4,1]$                \\ \bottomrule[1pt]
\end{tabular}%
}
\caption{MPO Decomposition Shape in T5 based and GPT based pre-trained language models}
\end{table}



\paratitle{Hardware}
We trained our model on four machine with 8 NVIDIA RTX3090 GPUs. For our base models, we adopt all these models released by Huggingface~\footnote{https://huggingface.co/}. 

\paratitle{Optimizer}
We used the Adam optimizer and vary the learning rate over the course of training. The vary
formula~\cite{vaswani2017attention} is follows in our work. We also used the $warmup\_steps = 500$.


\section{More Discussion}
\paratitle{Factorization Manner of MPO}
% 在这里我们讨论不同的MPO分解形式对MPOE结果的影响。
Here we discuss the effect of factorization manner of MPO decomposition on the MPOE results. 
As claimed in main text, the factorization manner of MPO is chosen by convenience due to fact due to that testing all possible decompostions is very time-consuming. 
In the viewpoint of entanglement entropy, that is controlled by the bond dimension $d_N$, as $d_N$ becomes larger, the entanglement entropy of the input data grasped by MPO grows accordingly and the accuracy is expected to be improved, thus $d_n$ will be more important as long as the network is away from underfitting. In other word, when $d_n$ becomes larger, different factorization manner should not make too much differences.
In our experiments, we do not truncate on the $d_n$, so we can assume that $d_n$ is large enough. Therefore different factorization forms have no effect on the robustness of the MPOE model.
Tabel show the results of our experiment on different factorization manner of MPOE,
where $n=3,5,7,9$ corresponding MPO structures are shown in Table~\ref{tab-factorization-mannner}.
As we have seen, all of these different factorization manner of MPO can efficient improve of the GPT model capacity. 

\begin{table}
\small
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccc} 
    \toprule[1pt]
        \multicolumn{1}{c}{\textbf{Experiments}} & 
        \begin{tabular}[c]{@{}c@{}} \\\textbf{PPL} \end{tabular} &  \begin{tabular}[c]{@{}l@{}}\textbf{WikiText}\\\textbf{BELU-2}\end{tabular} & \begin{tabular}[c]{@{}l@{}} \\\textbf{ BELU-4}\end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}\textbf{Avg.}\\ \#Pr/\#To(M) \end{tabular} \\ 
        \midrule[0.7pt]
        GPT-baseline & 21.27 & 28.69 & 9.46 & 124.4/124.4 \\
        MPOE(n=3) & 24.01 & 27.86 & 8.93 & 5.9/130.3 \\
        MPOE(n=5) & 20.72 & 28.77 & 9.48 & 32.9/157.4 \\
        MPOE(n=7) & 20.62 & 28.76 & 9.44 & 74.3/198.7 \\
        MPOE(n=9) & 20.78 & 28.45 & 9.38 & 157.1/214.6 \\
    \bottomrule[1pt]
\end{tabular}
}
\caption{Evaluation with different factorization manner.}
\label{tab-factorization-mannner}
\end{table}


\paratitle{Parameter Variation among Experts} 

\begin{table}
\centering
\small
\begin{tabular}{ccccc} 
\toprule
    \multicolumn{1}{c}{\multirow{1}{*}{Expert}} & \multicolumn{2}{c}{\multirow{1}{*}{Statistical Results}} & \multicolumn{2}{c}{\multirow{1}{*}{Variations Range}} \\
    Id &   Mea. & Std. Dev. & [0,1e-4) & [1e-4,1.5e-2) \\
    \midrule
        1                &1.39e-6 &0.030 & 50.15\% & 20.04\%\\
        2                &8.82e-6 &0.030 & 50.16\% & 20.07\%\\
        3                &3.74e-6 &0.031 & 50.19\% & 20.06\%\\
        4                &1.66e-5 &0.030 & 50.12\% & 19.67\%\\
        5                &6.62e-6 &0.031 & 50.18\% & 20.06\%\\
        6                &7.21e-6 &0.030 & 50.14\% & 20.06\%\\
        7                &1.02e-5 &0.030 & 50.16\% & 20.06\%\\
\bottomrule
\end{tabular}
\caption{Parameter variations between the first expert and each of the rest seven experts.}
\label{tab:parameter_var2}
\end{table}

In order to examine the information redundancy across experts, we first conduct an empirical study on how the learned parameters are different across different experts. 

Since there are no publicly available MoE-based Transformers  with learned parameters, we implement a MoE extension with eight experts based on the GPT2 model~\citep{radford2019language}, and fine-tune the model on the \emph{EMNLP news} dataset~\cite{EMNLPnews}. Then, taking the first expert as a reference, we calculate its parameter absolute difference (performing the subtraction between two corresponding entries of equal-sized matrices) with each of the rest seven experts, in mean and standard error. 

As we can see in Table~\ref{tab:parameter_var2}, more than 50.1\% of all the parameter differences is indeed very small, \ie $1e-4$. See appendix for more details on 
Such an observation indicates that there might exist redundant parameters across experts, which can be further  reduced or shared in the MoE architecture.    

\paragraph{Parameter Variations of GPT2+MPOE.}
% 为了说明我们的方法可以和MoE方法达到同样的效果，我们分别对比了MPOE与MoE微调之后不同和专家之间的差异。如表4所示，结果显示MPOE在微调之后的均值和标准差指标与MoE相近。我们也注意到4组expert均值差异更大，说明尽管我们控制了CT共享，训练AT确实学习到了“特定”类型数据的信息。这个结果说明，我们的方法确实以非常少参数以及相同的效果提升了模型的容量，进一步验证我们的方法的有效性。
To illustrate that our approach can achieve the same results as the MoE, we compared the differences between different experts after fine-tuning GPT2+MPOE and GPT2+MoE, respectively. As shown in Table~\ref{tab:parameter_var}, the mean and standard deviation metrics of GPT2+MPOE after fine-tuning are similar to those of GPT2+MoE. 
In addition, four groups of experts~(\ie 1,2,3,6) have a higher mean difference, indicating that the auxiliary tensors with limited parameters are able to learn more expert-specific knowledge.
This result demonstrates that our approach does enhance the capacity of the model with very few parameters as well as the same effect, further validating the effectiveness of our approach.



\begin{table}[h]
\centering
\small
\begin{tabular}{ccccc} 
\toprule
    \multicolumn{1}{c}{\multirow{1}{*}{Expert}} & \multicolumn{2}{c}{\multirow{1}{*}{Statistical Res.~(MoE)}} & \multicolumn{2}{c}{\multirow{1}{*}{Statistical Res.~(MPOE)}} \\
    Id &   Mea. & Std. Dev. & Mea. & Std. Dev.  \\
    \midrule
        1                &1.39e-6 &0.030 & 1.25e-5 & 0.011\\
        2                &8.82e-6 &0.030 & 1.82e-5 & 0.010\\
        3                &3.74e-6 &0.031 & 1.06e-5 & 0.013\\
        4                &1.66e-5 &0.030 & 1.56e-5 & 0.010\\
        5                &6.62e-6 &0.031 & 4.52e-6 & 0.012\\
        6                &7.21e-6 &0.030 & 9.65e-6 & 0.010\\
        7                &1.02e-5 &0.030 & 4.40e-7 & 0.011\\
\bottomrule
\end{tabular}
\caption{Parameter variations between the first expert and each of the rest seven experts based on GPT2+MoE and GPT2+MPOE architecture.}
\label{tab:parameter_var} 
\end{table}

\section{Maximum Mean Discrepancy among Experts} 
\label{appendix-mmd-in-experts}
In order to examine the information redundancy across experts, we first conduct an empirical study on how the output feature distribution are different across different experts. 
Since there are no publicly available MoE-based Transformers  with learned parameters, we implement a MoE extension with eight experts based on the T5 model~\citep{radford2018improving}, and fine-tune the model on the \emph{SST-2} dataset. 
% 然后，将相同的输入样本m输入到所有的专家中可以得到不同的输出特征。我们计算了不同特征之间的MMD，来观测这些输出特征在无穷阶距条件下是否服从相同的分布。MMD可以通过下面的公式计算：
Then, feeding the same number $m$ of input sample to all the experts can yield different output features. We computed the Maximum Mean Discrepancy~(MMD)~\cite{mmd2006GrettonBRSS} between different features to observe whether these output features follow the same distribution. The MMD can be computed by the following equation:
\begin{equation}
\small
    \rm{MMD}(\mathcal{F},X,Y) < 2\sqrt{K/m}(1+\sqrt{log\alpha^{-1}}),
    \label{eq:mmd}
\end{equation}
where the hypothesis test of level $\alpha=0.05$, $X,Y$ denote the different output feature among these experts, $m$ is the number of samples~($m=2500$ in our empirical study), $K=1$ is the kernel function.
% 我们将经验观测数值带入公式1中，可得不同的专家输出特征的MMD小于0.178时，可以认为专家输出特征在无穷阶距条件下服从相同的分布。
We can get different expert output features with MMD less than $0.178$ when we substitute the empirical observation values into Equation~\ref{eq:mmd}, and we can consider that the expert output features obey the same distribution.
% Then, taking the first expert as a reference, we calculate its parameter absolute difference (performing the subtraction between two corresponding entries of equal-sized matrices) with each of the rest seven experts, in mean and standard error. 
% 所有的MMD数值都小于0.178，这意味着这些专家的输出特征都服从相同的分布，换句话说，专家之间具有很多相似的信息。
As we can see in Figure~\ref{fig:layer0}, all the MMD values are less than $0.178$, which means that the output features of these experts all follow the same distribution.
Thus, we can share the information among these experts.

\begin{figure}[h!]
    \centering
    \small
    \includegraphics[width=0.5\textwidth]{image/appendix-fig/Layer_0.pdf}
    \caption{After increasing model capacity with the MoE framework for the T5 model~\cite{radford2019language}, the same inputs are used for eight experts, and the Maximum Mean Discrepancy~(MMD) of these expert output features are compared. According to the MMD defination~\cite{mmd2006GrettonBRSS}, it is obtained that different expert output features can be considered as the same distribution when the value of MMD is less than $0.178$. }
    \label{fig:layer0}
\end{figure}


% \bibliographystyle{acl_natbib}
% \bibliography{appendix}
